ReTracing: An Archaeological Approach Through Body, Machine, and Generative Systems

We present ReTracing, a multi-agent embodied performance art that adopts an archaeological approach to examine how artificial intelligence shapes, constrains, and produces bodily movement. Drawing from science-fiction novels, the project extracts sentences that describe human-machine interaction. We use large language models (LLMs) to generate paired prompts "what to do" and "what not to do" for each excerpt. A diffusion-based text-to-video model transforms these prompts into choreographic guides for a human performer and motor commands for a quadruped robot. Both agents enact the actions on a mirrored floor, captured by multi-camera motion tracking and reconstructed into 3D point clouds and motion trails, forming a digital archive of motion traces. Through this process, ReTracing serves as a novel approach to reveal how generative systems encode socio-cultural biases through choreographed movements. Through an immersive interplay of AI, human, and robot, ReTracing confronts a critical question of our time: What does it mean to be human among AIs that also move, think, and leave traces behind?

==> 2_overview.tex <==
\section{\modelab{} Overview}
\label{sec:overview}

In Nietzsche, Genealogy, History \cite{Foucault2001_nietzscheGenealogyHistory}, Michel Foucault writes: “The body is the inscribed surface of events (traced by language and dissolved by ideas), the locus of a dissociated self (adopting the illusion of a substantial unity)”. In generative AI models, language becomes the inscribing instrument: its prompts and negative prompts encode choreography into both body and code, translating fiction into movement and archiving its traces as data. Through this process, AI reimagines itself in the very gestures it generates and preserves—in being recorded, simultaneously dissolving the boundaries of its own identity.

\modelab{} explores how generative AI internalizes and reinforces biased models of embodied identity. Drawing from seven science fiction texts, the project extracts sentences that depict interactions between humans and machines. These literary descriptions, often infused with gendered affect and mechanical obedience, are processed by a large language model (LLM), which classifies them into two categories: prompts (what to do) and negative prompts (what not to do).


Here, AI "learns" to move not from sensor data or motion capture, but from the cultural and textual imagination encoded in fiction. The resulting prompt pairs are then routed through a diffusion-based network: human prompts are converted into short video clips using generative models \cite{wan2,qwen2}, visualizing plausible bodily postures; robot prompts are translated into precise motor commands on the control panel for a quadruped robot, which performs the same scripts within a mirrored environment.

These bodily movements performed by both human dancers and robotic agents are then captured using a multi-camera motion tracking system \cite{xiao2025spatialtrackerv23dpointtracking}. The output is a 3D digital dataset of movement traces, including point clouds, movement trails, and positional heatmaps. These traces are not just records of movement, but reflect how AI reinterprets literature into systems of behavioral constraint—capturing gestures of discipline, compliance, and control.




